Numerical Characterization of Fragmentation in Ionic Liquid Clusters

Ionic liquid ion sources are a promising technology that can be used for many applications from space propulsion to focused ion beam microetching. Ionic liquid ion sources produce ion beams by extracting single ions and metastable solvated ion clusters from the surface of the ionic liquid and accelerating them using an electric field generated by applying a voltage between a sharp tip and a plate with an aperture. The solvated ion clusters often fragment in the electric field region, reducing the specific impulse and efficiency for propulsion applications and increasing the beam spot size for focused ion beam applications. Fragmentation behavior has previously been characterized in the region with no electric field. However, fragmentation in an electric field has not been investigated as experimental results are difficult to interpret. The goal of this work is to use various numerical methods to characterize fragmentation under the effect of an electric field. Molecular dynamics simulations are performed of various ionic liquid clusters under different conditions to determine the rate of fragmentation. Physics-based models are compared to the molecular dynamics results with the goal of deriving a new model that accounts for the effect of the electric field on fragmentation. Approximate Bayesian computational methods are employed to infer the temperature of different ionic liquid cluster types and the percentage of the beam composed of each species by comparing simulated retarding potential analysis curves to experimental ones. Finally, the results of multi-scale N-body simulations are postprocessed and compared to experimental data. Results show agreement between experimental data and N-body simulations using the fragmentation rates determined by molecular dynamics.

==> signature.tex <==
% -*- Mode:TeX -*-
%
% Some departments (e.g. Chemistry) require an additional cover page
% with signatures of the thesis committee.  Please check with your
% thesis advisor or other appropriate person to determine if such a 
% page is required for your thesis.  
%
% If you choose not to use the "titlepage" environment, a \newpage
% commands, and several \vspace{\fill} commands may be necessary to
% achieve the required spacing.  The \signature command is defined in
% the "mitthesis" class
%
% The following sample appears courtesy of Ben Kaduk <kaduk@mit.edu> and
% was used in his June 2012 doctoral thesis in Chemistry. 

\begin{titlepage}
\begin{large}
This doctoral thesis has been examined by a Committee of the Department
of Chemistry as follows:

\signature{Professor XXX}{Chairman, Thesis Committee \\
   Professor of Chemistry}

\signature{Professor XXX}{Thesis Supervisor \\
   Associate Professor of Chemistry}

\signature{Professor XXX}{Member, Thesis Committee \\
   Haslam and Dewey Professor of Chemistry}
\end{large}
\end{titlepage}


